DisMix: Disentangling Mixtures of Musical Instruments for Source-level Pitch and Timbre Manipulation

Existing work on pitch and timbre disentanglement has been mostly focused on single-instrument music audio, excluding the cases where multiple instruments are presented. To fill the gap, we propose DisMix, a generative framework in which the pitch and timbre representations act as modular building blocks for constructing the melody and instrument of a source, and the collection of which forms a set of per-instrument latent representations underlying the observed mixture. By manipulating the representations, our model samples mixtures with novel combinations of pitch and timbre of the constituent instruments. We can jointly learn the disentangled pitch-timbre representations and a latent diffusion transformer that reconstructs the mixture conditioned on the set of source-level representations. We evaluate the model using both a simple dataset of isolated chords and a realistic four-part chorales in the style of J.S. Bach, identify the key components for the success of disentanglement, and demonstrate the application of mixture transformation based on source-level attribute manipulation.

==> sections/evaluation.tex <==
\section{Evaluation}
Disentanglement
- Given a mixture, randomly swap the timbre of each source-level DR for anything. Perform either single-source reconstruction or set-based reconstruction to evaluate whether the pitch is preserved and the timbre is swapped.
- Do the same but restrict the swapping for instruments belonging to the same SATB part. 
- Both cases evaluate disentanglement. While the first case emphasises on generalisability to out-of-distribution combinations of pitch and timbre, the latter is a more practical use case when it comes to music production whose performance should be better than the first case.

We also evaluate two approaches for reconstructing mixtures.
- Iteratively reconstruct a single source four times.
- Reconstruct the mixture in one pass of the decoder given a set of source-level DRs.
